Neural Network Guided Evolutionary Fuzzing for Finding Traffic Violations of Autonomous Vehicles

Self-driving cars and trucks, autonomous vehicles (AVs), should not be accepted by regulatory bodies and the public until they have much higher confidence in their safety and reliability -- which can most practically and convincingly be achieved by testing. But existing testing methods are inadequate for checking the end-to-end behaviors of AV controllers against complex, real-world corner cases involving interactions with multiple independent agents such as pedestrians and human-driven vehicles. While test-driving AVs on streets and highways fails to capture many rare events, existing simulation-based testing methods mainly focus on simple scenarios and do not scale well for complex driving situations that require sophisticated awareness of the surroundings. To address these limitations, we propose a new fuzz testing technique, called AutoFuzz, which can leverage widely-used AV simulators' API grammars to generate semantically and temporally valid complex driving scenarios (sequences of scenes). To efficiently search for traffic violations-inducing scenarios in a large search space, we propose a constrained neural network (NN) evolutionary search method to optimize AutoFuzz. Evaluation of our prototype on one state-of-the-art learning-based controller, two rule-based controllers, and one industrial-grade controller in five scenarios shows that AutoFuzz efficiently finds hundreds of traffic violations in high-fidelity simulation environments. For each scenario, AutoFuzz can find on average 10-39% more unique traffic violations than the best-performing baseline method. Further, fine-tuning the learning-based controller with the traffic violations found by AutoFuzz successfully reduced the traffic violations found in the new version of the AV controller software.

==> body/4_fuzzing_bck.tex <==
\section{AutoFuzz Methodology}
\label{sec:fuzzing}

Leveraging the grammar described above, this section describes \tool's test generation methodology in detail. We first give an overview of \tool and the definition of \bugs in our context (\cref{sec:overview}). \tool works in a blackbox evolutionary fuzzing setting. In the next two sections, we first discuss how evolutionary fuzzers work, in general (\cref{sec:theory}),  followed by how we realize \tool under this generic fuzzing framework for self-driving car domain (\cref{sec:main_algorithm}). % with different design choices. 


\subsection{\tool Overview}
\label{sec:overview}

Figure~\ref{fig:autofuzz_flowchart} shows a high-level overview of how  \tool works. \tool aims to test ego-car's controller in a blackbox manner.  The controller runs in the simulation environment and takes inputs from the simulator, \carla. \tool fuzzes in this input space. In particular, \tool generates different driving scenarios through \carla along which the controller can drive. 

To generate meaningful driving scenarios, we leverage \carla APIs, as discussed in~\Cref{sec:grammar}. \tool takes the API grammar as input and fuzz following the grammar spec. As a seed test case, the user selects a route map where the ego-car controller will drive and a seed scene, which is encoded as API grammar. Users can also optionally specify a search region and constraints. \tool uses these pieces of information to sample the input scenes. The simulator runs these scenes with ego-car controller under test to collect initial test cases and results. \tool uses these initial test cases and results to generate new test cases. The details of the new test cases generation procedure will be discussed in details in~\Cref{sec:main_algorithm}. New test cases will then be fed into the simulator to run. The found \bugs will be reported, and the results will be added to the test case collection. The iterative process will keep running until the time budget runs out.

% Figure \ref{fig:autofuzz_flowchart} shows a high-level overview of how  \tool works. \tool aims to test ego-car's controller, which is treated as a blackbox. The controller runs in the simulation environment and takes inputs from the simulator, \carla. \tool fuzzes in this input space. In particular, \tool generates different driving scenarios through \carla along which the controller can drive.

% To generate these scenarios, \carla exposes some APIs, which is encoded as test generation grammar, as discussed in Section 3. \tool takes such grammar as input and fuzz following the grammar spec. As a seed test case, the user selects a route map where the ego-car controller will drive and a seed scene, which is encoded as API grammar. Users can also optionally specify a search region and constraints, as discussed in Section 3. \tool uses these pieces of information to sample the input scenes. The simulator runs these scenes with ego-car controller under test to collect initial test cases and results. \tool uses these initial test cases and results to generate new test cases. The details of the new test cases generation procedure will be discussed in details in~\Cref{sec:main_algorithm}. New test cases will then be fed into the simulator to run. The found \bugs will be reported and the results will be added to test cases collection. The iterative process will keep running until the time budget runs out.

% \begin{figure}[t]
% \centering
% % url: https://drive.google.com/file/d/1MsJnf8ca4jks5KlUS5BHajweH8vFJ3XT/view?usp=sharing
% %\includegraphics[width=0.48\textwidth]{images/general/AutoFuzz_flow.pdf}
% %\includegraphics[width=\columnwidth]{images/general/AutoFuzz-Overview.pdf}
% \includegraphics[width=\columnwidth]{images/general/AutoFuzz-Workflow.png}
% %\vspace{-2mm}
% \caption{\small{\textbf{An illustration of how AutoFuzz works.}}}
% \label{fig:autofuzz_flowchart}
% \end{figure}


% \begin{figure}[t]
% \centering
% % url: https://drive.google.com/file/d/1MsJnf8ca4jks5KlUS5BHajweH8vFJ3XT/view?usp=sharing
% %\includegraphics[width=0.48\textwidth]{images/general/AutoFuzz_flow.pdf}
% \includegraphics[width=\columnwidth]{images/general/AutoFuzz-seed-selection.pdf}
% %\vspace{-2mm}
% \caption{\small{\textbf{Seed Selection \& Mutation Strategy per Generation}}}
% \label{fig:seed_selection}
% \end{figure}


\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/general/AutoFuzz-Workflow.png}
         \caption{High-level Workflow}
         \label{fig:workflow}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/general/AutoFuzz-seed-selection.pdf}
         \caption{Seed Selection \& Mutation Strategy per Generation}
         \label{fig:mutation}
     \end{subfigure}
        \caption{\small{\textbf{An illustration of how AutoFuzz works}}}
        \label{fig:autofuzz_flowchart}
\end{figure*}

%Within this framework, now we will describe how different fuzzing components are designed. 

\subsubsection{Traffic Violations}

%\noindent\textbf{Bug Types}
%There are many kinds of erroneous behaviors a self-driving car can potentially have \cite{}. 
% \noindent
% \textbf{Traffic Violations.} 
Here, we focus on three types of violations: collision, going out-of-road and running red light since these three can lead to serious consequences. 
%The first two were previously studied in the literature~\cite{misbehavior}. 
A {\em collision} consists of colliding with other vehicles, cyclists/motorcycles, pedestrians, or stationary objects. % like a trash can or a road boundary.
An {\em out-of-road} violation consists of going to a wrong lane (a lane that has opposite traffic direction that the car drives towards) and going off-road. 
%We will later present how we formulate objectives to promote finding such violations.
%Note that, our framework can be easily extended for other types of violations, e.g., running a stop sign. 


% \noindent
% \textbf{Unique Violations.} 
The goal of a good fuzzer should be to find diverse types of bugs. However, defining distinct \bugs in our case is a hard problem. Merely comparing the violation-inducing inputs will lead to infinitely different violations. For example, let's assume that a static object (say, a barrel) in front of a car causes a crash. By modifying unrelated input parameters (e.g., the position of another pedestrian, the color of another vehicle, etc.) that are out of the vision of the ego-car controller, we can generate an infinite number of {\em different} violations. Clearly, such repetitive violations are not interesting. Thus, a criterion defining unique \bugs is needed.

% Abdessalem \etal~\cite{testing_vision18} define that two test scenarios are distinct if they differ in "the value of at least one static variable or in the value of at least one dynamic variable with a significant margin." This definition fails in our more complex high-dimensional scenarios, as the example above will be considered different bugs by their criteria. To avoid counting similar bugs as different bugs, we give a definition that gives a "lower bound" of the number of bugs by binning them. Two bugs caused by two input scenes x and y are distinct if the bugs are of different categories (e.g., collision vs. out-of-road) or the distance between x and y is greater than some threshold.  In this work, we chose two bugs to be distinct if they have at least p\% fields being different\textemdash for a discrete field the corresponding values should be different, and for a continuous field, the corresponding values should be different by a margin as large as q\% of $max-min$ where $min$ and $max$ are the boundary values of the field.~\bray{check this} For example, a car of red color and a car of blue color have different "color" field. When the initial speed range for a car is $[0,10]$ m/s, If in bug A, this car has initial speed 3 m/s while in bug B the car is with initial speed 4 m/s, then this field is considered the same between the two bugs since $\frac{4m/s-3m/s}{10m/s-0m/s}=0.1<0.15$. 

Abdessalem \etal~\cite{testing_vision18} define that two test scenarios are distinct if they differ in "the value of at least one static variable or in the value of at least one dynamic variable with a significant margin." This definition fails in our high-dimensional scenarios, as the example above will be considered different violations by their criteria. To address this issue,  we count the number of unique violations as follows: 

\noindent
\textit{{\bf Unique Traffic Violations}: Under a given type of traffic violation (collision or out-of-road), two violations caused by input scenes x and y are {distinct} if at least $th_1\%$ of the total number of changeable fields (with range larger than 0) are different between the two, where $th_1$ is a configurable threshold.
}

% \textit{
% %Two violations caused by input scenes x and y are {distinct} if the violations are of different categories 
% %(e.g. collision vs. out-of-road) or at least $th_1\%$ of the total number of changeable fields (with range larger than 0) are different between the two, where $th_1$ is a configurable threshold.
% Under a given type of traffic violation (collision or out-of-road), two violations caused by input scenes x and y are {distinct} if at least $th_1\%$ of the total number of changeable fields (with range larger than 0) are different between the two, where $th_1$ is a configurable threshold.
% } 

For a discrete field, the corresponding values are different if they are non-identical in $x$ and $y$ (\eg ``color" field is different between a red and a blue car). 
For a continuous field, the corresponding normalized values should be distinguishable by at least $th_2\%$, where  $th_2$ is a user defined threshold. 
Here normalized field value is computed \wrt its allowable range. %, \ie $max-min$. 
For instance, if the speed range of a car is $[0,10]$m/s, and two violations occur at speeds 3m/s and 4m/s, the field is considered to be same between the two violations since $\textstyle \frac{4-3}{10-0}=0.1<0.15$, where $th_2=0.15$. 

%Within this framework, now we will describe how different fuzzing components are designed in details. 

\subsection{Fuzzing Theory}% and Motivation}
\label{sec:theory}

The goal of any \textit{evolutionary fuzzers} (\GF) is to maximize the number of bugs found within a given resource (e.g., time). Therefore, \GF can be thought of an optimization problem, where it searches over the entire input space to maximize bug count, \aka \bug, in our  case. More formally,  if \allx is the space of all possible inputs to a program, a \GF tries to search over \allx to maximize \bug count (\ally) within a fixed budget, say $\mathcal{T}$. 
%Thus, if $B_t$ is the set of bugs found by input $x_t\in\mathcal{X}$ at fuzzing step $t$,  then \GF  can be formally represented as:
Thus, if $B_t$ is the set of \bugs found by input $x_t\in\mathcal{X}$ at fuzzing step $t$, 
%and {\em objective function} $f: x_t\rightarrow B_t$ maps inputs ($x_t$) to bug count $B_t$ such that if $f(x)$ decreases bug count increases, 
then \GF can be formally represented as: $\scriptstyle{\mathcal{Y_\mathcal{T}} =
    \max\norm{~\bigcup_{t=1}^\mathcal{T} B_t}}$.
% %$\scriptstyle{\mathcal{Y_\mathcal{T}} = \max\norm{~\bigcup_{t=1}^\mathcal{T} B_t  }
% %                = \max_{x_t\in\mathcal{X}}\norm{~\bigcup_{t=1}^\mathcal{T} f(x_t)}}$.
% % 
% \begin{equation}
% \scriptstyle
%     \setlength{\abovedisplayskip}{0pt}
%     \setlength{\belowdisplayskip}{0pt}
%     \label{eq:formal_main_0}
%     \mathcal{Y_\mathcal{T}} =
%     \max\norm{~\bigcup_{t=1}^\mathcal{T} B_t  }
%               % = \min_{x_t\in\mathcal{X}}\norm{~\bigcup_{t=1}^\mathcal{T} f(x_t)}
% \end{equation}
% 
Here $\scriptstyle \|\cdot\|$ represents the norm and $\scriptstyle{\bigcup(\cdot)}$ represents the union of all elements.

% ~\eq{formal_main_0} 
% indicates that minimizing the union of $f(x)$ happens over all possible inputs. 
% Since the input space \allx in our case is prohibitively large, an exhaustive search to maximize the equation 
% is infeasible. 
% Instead, one needs to identify and focus the search on promising regions that will maximize the number of bugs found.  
% To identify such promising inputs, most \GF generates mutated inputs; 
% The mutation process is the key to a fuzzer's effectiveness. Ideally, fuzzers want to spend more mutations in parts of the program input space that are likely to result in higher bug count.  
% In fact, most of fuzzing research effort has been spent on designing different mutation strategies based on different information sources (\eg input formatting~\cite{godefroid2017learn}, rare branches~\cite{lemieux2017fairfuzz}, \etc) to focus more on the promising input regions and fine-tune the corresponding parameters. A mutation strategy determines how mutation occurs, this depends on finding optimal values for three main {\em mutation parameters}:

% \squishlist
% \item[(i)] \textit{Input ($x\in$\allx)}: which inputs to mutate~\cite{bohme2017coverage}?  
% \item[(ii)] \textit{Mutation location ($ml$)}: which locations in each input to mutate~\cite{lemieux2017fairfuzz, vuzzer,chen2018angora, steelix,You2019SLFFW,You2019ProFuzzerOI}?  and 
% \item[(iii)] \textit{Mutation operator ($mo$)}: the mutation operation to perform on those locations, \ie, which new values should replace the old values~\cite{she2018neuzz, chen2018angora, vuzzer}? 
% \squishend

The above equation indicates that maximizing the union of $B$ happens over all possible inputs. Since the input space \allx in our case is prohibitively large, an exhaustive search to optimize the equation is infeasible. 
Instead, one needs to identify and focus the search on promising regions to optimize the number of violations found.  
To identify such promising inputs, most \GF generates mutated inputs; 
The mutation process is the key to a fuzzer's effectiveness. 
Ideally, fuzzers want to spend more mutations in parts of the program input space that are likely to result in higher violation count. 
Thus, the success of fuzzing depends on designing the following three parts:

\squishlist
\item[(i)] \textit{Seed Selection ($x\in$\allx)}: which inputs to mutate~\cite{bohme2017coverage}?  
\item[(ii)] \textit{Mutation($m$)}: which locations in each input to mutate~\cite{lemieux2017fairfuzz, vuzzer,chen2018angora, steelix,You2019SLFFW,You2019ProFuzzerOI} and with what value~\cite{she2018neuzz, chen2018angora, vuzzer}?  and 
\item[(iii)] \textit{Objective function ($F$)}: How to design a objective function to maximize the \bug count? 
\squishend


Thus, given an input $x_{t-1}$ at step $(t-1)$, the next generated
input $x_{t}$ depends on $x_{t-1},m$. %\bray{what are the subscript of m\_l and m\_o ?}
The set of \bugs $B_t$ found by $x_t$ can be represented as a function ($F$) of these fuzzing parameters, i.e.,~$B_t=-F(x_{t-1},m)$, such that minimizing $F$ will maximize the \bugs. 
Thus, \GF can be written as: 
{
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\begin{equation}
    \label{eq:formal_main}
    \scriptstyle
    %\vspace{-2mm}
    \mathcal{Y_\mathcal{T}} 
    %= \maximize_{x,ml,mo}\norm{~\bigcup_{t=1}^\mathcal{T} E_t}  
    = \min_{x_{t-1},m}\norm{~\bigcup_{t=1}^\mathcal{T}F(x_{t-1},m)~}
\end{equation}
}
Note that, in the above equation, $x_0$ is an initial seed input. The function $F$ is often used to optimize a proxy of bug count as number of bugs in a program may not be known beforehand. For example, traditional greybox fuzzers use edge-coverage~\cite{zalewski2017american} of traditional programs to approximate bug count. 
In the rest of this section, we will discuss how \tool realizes this optimization (\eq{formal_main}) for self-driving car domain. 




\subsection{Evolutionary Algorithm with Gradient Guided Mutation}
\label{sec:main_algorithm}
As discussed in~\Cref{sec:theory}, \tool makes three choices \wrt designing objective functions, mutation strategy, and seed selection. 
We discuss these designs in details.   

\subsubsection{Objective Function}
As discussed in~\Cref{sec:theory}, 
we formulate fuzzing as an optimization problem, where a fuzzer tries to find optimal values of a given objective function ($F$ in \Cref{eq:formal_main}). 
The ultimate objective of any fuzzing algorithm is to maximize bug count. 
% However, if directly counting the bug is not possible, or costly, a common practice is to propose an alternate objective function, which can approximate the bug count.
However, directly optimizing for maximizing bug counts may not be efficient especially in cases where bugs are relatively rare. A common practice is to propose an alternative objective function for optimization.  
In our case, we define the following objective functions:


{
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\vspace{1mm}
\centering
\footnotesize
\begin{tabular}{lll}
\toprule
\textbf{Violation} &  &  \\ 
\textbf{Type} & \textbf{Objective}  & \textbf{Definition} \\ \toprule
 \multirow{3}{*}{Collision} &   $F_{collision}$ &:= \textrm{speed of ego-car at collision} \\
    & $F_{object}$ &:= \textrm{minimum distance to other objects} \\ 
    & $F_{view}$ &:= \textrm{minimum angle from camera's view} \\ \midrule
\multirow{3}{*}{Out-of-road}    & $F_{wronglane}$ &:= \textrm{minimum distance to an opposite lane} \\
    & $F_{offroad}$ &:= \textrm{minimum distance to a non-drivable region} \\
    & $F_{deviation}$ &:= \textrm{maximum deviation from interpolated route} \\ \midrule
\multirow{1}{*}{Red Light} & $F_{redlight}$ &:= \textrm{violation of running red light} \\ \bottomrule
\end{tabular}
\vspace{1mm}
}


We choose all of these functions except $F_{redlight}$ to be continuous for a smooth optimization of the search algorithm. 
In particular, the first three, $F_{collision}$, $F_{object}$, and $F_{view}$, promote collision. Similar objectives were proposed in \cite{testing_vision18, nsga2nn}. $F_{collision}$ and $F_{object}$ promote the severity of collision and the chance of collision, respectively. $F_{view}$ promotes cases where the object(s) involved are within the camera(s) view. Note a special case of $F_{object}$ is the minimum distance between either of the front two corners of the ego-car's bounding box and any other object's corner of bounding box. This special case can be used for testing controllers that only have front camera(s) since it might not be fair to test out-of-sight collision which goes beyond their assumed capability. 

$F_{wronglane}$, $F_{offroad}$, and $F_{deviation}$ promote out-of-road error. $F_{wronglane}$ promotes going to wrong lane and $F_{offroad}$ promotes going off road, while $F_{deviation}$ promotes both. Figure \ref{fig:wronglane_objective} illustrates an ego-car driving along a road. The angle between the ego-car's forward direction and the lane center is denoted $\Theta$ and the ego-car's center's distance from the lane center is denoted $d_{dev}$. $F_{deviation}$ is defined to be the product of the two i.e. $F_{deviation}=\Theta \times d_{dev}$.
% the angle between the two vectors is denoted as $\theta$ (in radian); $F_{wronglane}=||d||_2\times (1-\frac{2\times\theta}{\pi})$. 
$F_{wronglane}$ and $F_{offroad}$ measure the ego-car's distance from the closest lane of opposite direction or non-drivable region. In particular, $F_{wronglane}$ is the minimum of $d_{forward}$, $d_{roadleft}$, $d_{egoleft}$, $d_{roadleft}$ and $d_{egoleft}$, which (the later two are not shown in the figure) denote the ego-car's distance along different directions \wrt the closest point that is on a road with different direction. $F_{offroad}$ is defined similarly except the closest point will be the one that is off road rather than on a opposite direction road.

Lastly, $F_{redlight}$ indicates whether the car indeed runs a red light and promotes running red light error. In future work, it can also be made continuous. For example, it can be the time it takes from ego-car crosses the stop line and the traffic light turns red.

\begin{figure}[ht]
\centering
% url: https://drive.google.com/file/d/1MsJnf8ca4jks5KlUS5BHajweH8vFJ3XT/view?usp=sharing
\includegraphics[width=0.2\textwidth]{images/general/wronglane_objective.pdf}
\caption{\textbf{\small{Parameters computing the wrong lane objective function}}}% $\pmb{F_{wronglane}}$.}}}
\label{fig:wronglane_objective}
\end{figure}

\noindent
\textit{Single-Objective Optimization.}
We formulate the fuzzing problem as a constrained single-objective optimization problem. 
Let $x$ be an input, \ie, a scene with all the searchable fields. 
Denote $F_i(x)$ for $i=1,...,n$ to be $n$ objective functions, $w_i$ to be some user provided weights, 
and $g_j(x)$ for $j=1,...,p$ to be $p$ constraints, where each constraint is expressed as $\leq$  $0$ form. Then, the objective function $F(x)$ of ~\Cref{eq:formal_main} can be expressed in constrained weighted sum as: $\textstyle   \textrm{min}_x~\sum_{i=1}^{n} w_i F_i(x), 
    \textrm{s.t. } g_j(x) \leq 0 ~\forall j=1,...,p$.
Note that the reason we use a weighted sum single-objective optimization rather than multi-objective optimization as in \cite{testing_vision18, interactiontest, nsga2nn} is that our goal is to find maximum number of unique \bugs rather than \bugs that have the best pareto-front of multiple objectives. 
% \begin{align*}
%     \textrm{min}_x~ & \sum_{i=1}^{n} w_i F_i(x) \\ 
%     \textrm{s.t. } & g_j(x) \leq 0 ~\forall j=1,...,p
%     \label{eq:optimization}
% \end{align*}

% \ziyuan{why you formulated it as minimization as opposed to maximization? It'd be better to stick to max following~\Cref{eq:formal_main}}. \bray{mutl-objective optimization usually use minimization by convention. The GA package I used, the ICSE paper, and wikipedia page all seem to use minimization.}
%Note that, in order to maximize bug count (objective $F$ in~\Cref{eq:formal_main}), we need to minimize the objectives used for Collision and Out-of-Road bugs. For example, 

% There are many kinds of algorithms we can potentially use to solve it e.g. multi-objective genetic algorithms \cite{}, bayes optimizations \cite{}. In this work, we mainly focus on NSGA2 \cite{nsga2} and NSGA2-DT \cite{testing_vision18}, as they have been shown to be effective on a smaller-scale similar error finding optimization problem. Our framework can be easily extended to also support other multi-objective optimization algorithms.






% \ziyuan{I am not sure whether we need to talk about constraint again.}
% \paragraph*{constraints} As mentioned in~\Cref{sec:grammar}, \tool grammar allows two kinds of constraints: individual variable constraints and joint constraints. For each field $x_i$, its individual constraints is defined as its possible minimum and maximum values. Each joint constraints is defined as an inequality equation $\sum_{i\in \mathbf{S}} c_i \times x_i \leq v$, where $S$ is a subset of all features, $c_i$ is a real number coefficient, and $v$ is a real value. Users can specified both as discussed earlier. \tool will respect both but in a different way. It will clip the values for individual variable constraints' violations, while it will avoid running simulation for cases that violate joint constraints.



% \subsection{Test-Case Distillation.}
% Defining distinct bugs in self-driving car controller is a very hard problem. Bugs in self-driving car controller are different from traditional software bugs. Because there are many dimensions of the input parameters being continuous, there can be infinitely "different" bugs. For example, let's assume that the existence of a static object (say, a barrel) in front of a car causes a crash. By modifying other input parameters (e.g. the position of another pedestrian, the color of another vehicle etc.) that are probably unrelated (e.g. they may not be seen by a pure camera-based controller), we can get an infinite number of "different" bugs that provide little extra information. Thus, a criteria defining distinctness of bugs is needed.

% In \cite{testing_vision18}, they define that two test scenarios are distinct if they differ in "the value of at least one static variable or in the value of at least one dynamic variable with a significant margin." This definition fails in our more complex scenarios as the aforementioned example will be considered different bugs by their creteria. To avoid counting similar bugs as different bugs, we give a definition that gives a "lower bound" of the number of bugs by binning them.
% \begin{definition}
% Two bugs caused by two seed scenes x and y are considered distinct if they are either of different categories (e.g. collision VS out-of-road) or
% \[
% f(x_{int}, y_{int}) + g(x_{real}, y_{real}) > th 
% \]
% where $f$, $g$ are two distance functions, $x_{int}$ and $x_{real}$ are the int fields and real fields of $x$, respectively. $y_{int}$ and $y_{real}$ are defined similarly. $th$ is a non-negative threshold.
% \end{definition}
% In this work, for simplicity, we let $f$ to be the $l_0$ norm and let $g$ to be the sum of the element-wise 0-1 step function with threshold at 0.15 after normalizing the field. We also let $th$ to be equal to half of $||x||_0$ which is the number of fields a seed scene has. In other words, two bugs are considered distinct if they have at least 50\% fields being different (for discrete fields) or different by a large margin (for continuous fields).

\begin{algorithm}
    \scriptsize
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{sampling(), evaluate(), max-gen, pop-size, generation-to-use-DNN, candidate-multiplier, max-mating-iter, gradient-mutation-parameters}
    \Output{unique-bugs}
    
    initial-population = sampling(pop-size)\;
    initial-unique-bugs, initial-objectives = evaluate(initial-population, [])\;
    
    
    generations = 1\;
    all-population = initial-population\;
    all-objectives = initial-objectives\;
    unique-bugs = initial-unique-bugs\;
    
    current-population, current-objectives = initial-population, initial-objectives\;
    
    \While {generations < max-gen}{
        mating-iter = 0;
        candidate-offspring = []\;
        remaining-size = pop-size $\times$ candidate-multiplier\;
        \While {mating-iter < max-mating-iter and remaining-num > 0}{
            mating-iter += 1\;
            parents = selection(current-population, remaining-num)\;
            new-candidate-offspring = crossover(parents)\;
            new-candidate-offspring = mutation(new-candidate-offspring)\;
            new-candidate-offspring = filtering(new-candidate-offspring, candidate-offspring, unique-bugs)\;
            
            candidate-offspring = merge(candidate-offspring, new-candidate-offspring)\;
            remaining-num = pop-size - len(candidate-offspring)\;
        }
        \If {remaining-num > 0}
        {
            remaining-candidate-offspring = sampling(remaining-num)\;
            candidate-offspring = merge(candidate-offspring, remaining-candidate-offspring)\;
        }

        \If {generations > generation-to-use-DNN}
        {
            \textcolor{blue}{f = train-DNN(all-population, all-objectives)}\;
            \textcolor{blue}{sorted-candidate-offspring = rank-by-confidence(candidate-offspring, f)}\;
            \textcolor{blue}{offspring = select(sorted-candidate-offspring)}\;
            \textcolor{red}{offspring = constrained-gradient-guided-mutation(offspring, f, gradient-mutation-parameters)}\;
        }
        
        new-unique-bugs, new-objectives = evaluate(offspring, unique-bugs)\;
        
        all-population = merge(all-population, offspring)\;
        all-objectives = merge(all-objectives, new-objectives)\;
        unique-bugs = merge(unique-bugs, new-unique-bugs)\;
        
        combined-population = merge(current-population, offspring)\;
        combined-objectives = merge(current-objectives, new-objectives)\;
        
        current-population, current-objectives = survival(combined-population, combined-objectives, pop-size)\;
        
        generations += 1\;
    }
    
    
    \Return unique-bugs
    

    \caption{\textbf{\small{\GAUNNNGRAD}}}
    \label{alg:ga-un-dnn-adv}
\end{algorithm}



\smallskip
\subsubsection{Base Genetic Algorithm for Candidate Test Cases Generation}
%For mutation strategy, 

We use a base genetic algorithm to generate new candidate test cases. In particular, at each generation, the genetic algorithm takes in all the test cases with results so far, selects parent test cases, and generates new candidate test cases through crossover and mutation. We adapt some choices of selection, crossover, and mutation from \cite{nsga2, testing_vision18, nsga2nn}. The details of each part is as the following.

\noindent \textbf{Sampling} (line 1): For generating one instance, we randomly sample each field according to its user-specified search range and distribution. If the specified constraints are not satisfied, each variable will be re-sampled. If the specified constraints have very few small probabilities and cannot be satisfied after trying a specified number of attempts, the program will stop and raise an error. 

%Note that we apply duplicates elimination (discussed below) within the generated instances to ensure the diversity of the initial population.
 
\noindent \textbf{Selection} (line 13): 
We adopt binary tournament selection with a replacement, as per original \NSGA implementation~\cite{nsga2}. It creates two duplicates for each sample and randomly pair up these new samples. It chooses each pair's winner and randomly pair them up as the parents for this generation's mating process. The rank of two individuals will be purely determined by the objective function described in the previous subsection.

\noindent \textbf{Crossover} (line 14): Simulated Binary Crossover \cite{SBX}, a classical crossover method commonly used for float points, is adopted. A distribution index ($\eta$) is used to control the similarity of the offsprings and their parents. The larger $\eta$ is, the more similar the offsprings are \wrt their parents. We set $\eta=5$ and probability=$0.8$ to allow more diversity of offsprings.

\noindent \textbf{Mutation} (line 15): Polynomial Mutation is applied to each discrete and continuous variable~\cite{polymutation}. For discrete variables, we treat the value as continuous during the mutation and round them afterwards. We clip the values at specified minimum and maximum values. Following \cite{testing_vision18}, mutation rate is set to $\frac{5}{k}$, where $k$ is the number of variables per instance. The mutation magnitude is controlled by a variable $\eta_m$. Based on \cite{polymutation}, $\eta_m$ usually induces a perturbation $\textstyle O(\frac{x_{i_{max}}-x_{i_{min}}}{\eta_m})$, where $x_{i_{max}}$ and $x_{i_{min}}$ are the upper and lower bounds of a variable $x_i$.  We set $\eta_m=5$ to promote larger mutations.

\noindent \textbf{Duplicates Elimination} (line 16): 
After each selection, crossover, and mutation, the proposed offspring are filtered out if they are similar to any previous relevant \bugs. The mating will rerun until the number of offspring reaches the number of desired population size or maximum number of iterations reaches. Similar tracking method was used in \cite{interactiontest} for different purpose. They used a cache to store the best solutions so far while here we record detected unique \bugs to sample / mutate test cases to the extent of being distinct enough from found unique \bugs.





% Each configuration's score is a weighted sum of the objective functions. Given a configuration $x$, it has score
% \[
% score(x) = \mathbf{w} \cdot \mathbf{F}(x),
% \]
% where $\mathbf{w}$ is the user's provided weight and $\mathbf{F}(x)$ is the objective values collected from running simulation of the configuration $x$. This score is used to rank configurations during the genetic search algorithm. 


\subsubsection{Proxy DNN for Seed Filteration and Gradient-Guided Mutation}
Evolutionary Algorithm tends to suffer from slow convergence but in our case simulations are expensive to run. Thus, to further improve the efficiency of the search process, we actively train a DNN at each generation after the initial test cases collection stage to help selecting and further mutating candidate test cases generated by the genetic algorithm. Note that previous work \cite{nsga2nn} also leverages a DNN to help selecting test cases. There are several major differences. First, we train a single DNN for a binary classification of \bug rather than several DNNs for regressing over all objective values as in \cite{nsga2nn}. It follows that we rank test cases based on confidence value of being a \bug rather than the pareto front from multiple DNNs. This design choice is because our goal is to find maximum number of valid, diverse \bugs rather than finding \bugs achieving optimal multiple objectives at the same time. Second, we actively train the DNN along the genetic algorithm search process rather than training fixed ones at the beginning. This active training procedure leads to two benefits: less initial population and improved approximation over time. We show both design choices introduce performance gains in the experiment section. 


\noindent \textbf{DNN Filteration} (line 25-27): 
The DNN is trained using previous runs results to predict if a test case leads to a \bug or not. The trained DNN is then used to rank all the candidate test cases generated by the genetic algorithm based on the confidence of leading to a \bug. The top test cases which are considered more likely to cause \bugs are selected. 

\noindent \textbf{DNN Gradient-Guided Mutation} (line 28): 
We apply constrained gradient guided mutation on these selected top candidate test cases to maximize their likelihood of leading to \bugs further. The procedure is shown in \ref{alg:attack}. It is adapted from the constrained adversarial attack in \cite{constrainedpgd}. 

\begin{algorithm}
    \scriptsize
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{$x$: test cases, $f$: DNN forward function, $th_1$: threshold of conducting a perturbation, $th_2$: threshold of stopping a perturbation, $n$: maximum number of iterations, $\lambda$: step size, $c$: constraints, $\epsilon$: maximum perturbation bound}
    \Output{$x'$: mutated test cases}
    
    $x' = x$\;
    $i = 0$\;
    \If {$f(x)>th_1$}{
        return $x$\;
    }
    
    \While {$i < n$}{
        $i+= 1$\;
        $dx$ = $\lambda \frac{df(x')}{dx'}$\;
        $x' = x' + dx$\;
        $dx = clip(x' - x, \epsilon)$\;
        
        \If {check-constraint-violation ($c$, $dx$) == True}{
            $dx$ = linear-regression ($c$, $dx$)\;
        }
        \If {is-similar ($X$, $x+dx$)}{
            break\;
        }
        $x' = x + dx$\;
        
        \If {$f(x') > th_2$}{
            break\;
        }
    }
    
    
    \Return $x'$
    

    \caption{\textbf{\small{constrained gradient guided mutation}}}
    \label{alg:attack}
\end{algorithm}


The procedure is iterative. A test case $x$ is only perturbed when its DNN confidence of leading a \bug i.e. $f(x)$ is larger than a threshold $th_1$. This is because if a test case is already considered to be highly likely to lead to a \bug, there is no extra benefit of further perturbing it. Otherwise, an iterative process (line 6-20) begins. At each iteration, a small perturbation $dx$ will be generated (line 8) via back-propagation from maximizing the test case's DNN confidence of leading a \bug . The perturbation is then clipped based on a user specified maximum perturbation bound $\epsilon$ (line 9-10). Next, the perturbation will be checked against constraint violation (line 11). If a violation happens, a linear regression is applied to project it back to being within the constraints. The perturbed test case is then checked against previously found \bugs (line 14) . If a similar case is found, the perturbation process will end and the latest perturbation won't be applied. Otherwise, the current perturbation is applied on top of the perturbed test case from last iteration (line 17). The new perturbed test case is then fed into DNN to get its confidence of leading a \bug. If this confidence is larger than a specified threshold $th_2$, the mutated test case will be returned and the mutation procedure will end. Otherwise, a new iteration will begin. 


Note that one difficulty here is to make sure the perturbed test case still satisfy the user defined constraints. The simplest solution is to stop the perturbation before the step that leads to a violation. When the constraints are linear, however, one can do much better. One insight is that if the unperturbed test case satisfies constraints and its perturbation satisfies the constraints as well, then the perturbed test case also satisfies the constraints. Thus, only the perturbation needs to be checked against the constraints after each step. If some constraints are violated, a linear regression can be applied to the perturbation, where non-constant part of the constraints are weights, test case is the variable and constant part of the constraints are the objectives, to project the perturbation back to being within the boundary. In contrast to the method proposed in \cite{constrainedpgd}, where the constraint matrix is simplified to a reduced echelon form and some variables are considered dependent and thus directly assigned values according to the simplified constraint matrix and the independent variables' values, using linear regression can give the closest point on the boundary to the proposed perturbed test case.








% We adapt the Non-dominated Sorting Genetic Algorithm version 2 (\NSGA) \cite{nsga2} algorithm, a widely used evolutionary algorithm for multi-objective search~\cite{testing_vision18}.  \NSGA~\cite{nsga2} follows the generic procedures of a genetic algorithm with a modified mating and survival selection steps. First, individuals are selected based on Pareto-frontiers. 
% To split a frontier item, %When it comes to a front that needs to be split,
% individuals with larger crowding distance are selected. A test case's crowding distance is the manhattan distance with its neighbors in the objective space with boundary points having infinite distance. 
% To increase selection pressure, \NSGA uses a binary tournament mating selection. In particular, every pair of two individuals are first compared by rank and then crowding distance.

% Here we want to find distinct \bugs. Hence, we don't want the algorithm to be too greedy and adapt \NSGA by adding a duplicate elimination mechanism that allows more diversity. Algorithm \ref{alg:ga-un-dnn-adv} shows our version (\NSGAUN) in  details.


%our algorithm NSGA2-UN. 
%It worth noting that it is easy to extend our framework to support other algorithms.

%We adapt the Non-dominated Sorting Genetic Algorithm version 2 (NSGA2) \cite{nsga2} algorithm, which is a widely used evolutionary multi-objective search algorithm and also used in \cite{testing_vision18} for our framework since it has been shown before that it can effectively find bugs for testing an Automated Emergency Braking system in a simple one pedestrian crossing street scenario. NSGA2\cite{nsga2} follows the general procedures of a genetic algorithm with a modified mating and survival selection steps. First, individuals are selected based on Pareto-frontiers. When it comes to a front that needs to be split, individuals with larger crowding distance are selected. A test case's crowding distance is defined to be the manhatten distance with its neighbors in the objective space. The boundary points for each objective is considered to have crowding distance infinity. To increase selection pressure NSGA2 uses a binary tournament mating selection. In particular, every pair of two individuals are first compared by rank and then crowding distance.



% In our case, since we want to find cases that are very distinct with each other, we don't want the algorithm to be too greedy. Thus, we adapt NSGA2 by adding a duplicate elimination mechanism that allows more diversity. Algorithm \ref{alg:ga-un-dnn-adv} shows our algorithm NSGA2-UN. It worth noting that it is easy to extend our framework to support other algorithms.







% \ziyuan{we probably do not need to say this again?}
% \noindent \textbf{Fitness Functions}: We use the summation of the objective functions defined in the earlier section as the fitness function. The weights can be adjusted according to a user's need. For example, if the user only wants to focus on finding collision errors, the last three weights can be set to 0.



% \noindent \textbf{Survival} (line 11):
% We use \NSGA's default survival strategy, rank and crowding survival, and only keep the initial population size (\ie we cut off half of data from the parents and offspring combined set). It first ranks the data based on pareto-frontier, %non-dominated sort the data, 
% it then includes front by front until coming to a front that it has to split. 
% It takes the elements of that particular front based on crowding score.

% $l_p$-norm distance (after normalization of each continuous field and counting discrete field difference as t ($0\leq t\leq 1$) which trades off importance of continuous and discrete field)) is larger than a threshold value $th$.

    





==> body/methodology.tex <==

%\section{The Language}
\section{Processing API Specifications}


\subsection{Grammar Overview}
%Listing \ref{lst:grammar} shows the grammar of our proposed language. 
\lang allows developers/testers to express a starting scenario, crash triggering situation, and other output conditions that need to be maintained while simulating crashes. 

%\begin{lstlisting}[float,caption={Simplified Grammar Regular Grammar (RG) with tail recursion for autonomous driving test case generation.},captionpos=b,mathescape=true,frame=single,belowskip=-\baselineskip,label={lst:grammar}]

\begin{figure}[ht]
\centering
% url: http://draw.accidentsketch.com/
\includegraphics[width=0.4\textwidth]{images/general/AutoFuzz-Page-3.pdf}
\caption{A simplified version of CARLA APIs under test}
\label{fig:test_case_demo}
\end{figure}

\begin{lstlisting}[float,caption={Simplified Grammar (G) for autonomous driving test case generation.},captionpos=b,mathescape=true,frame=tb,belowskip=0pt,basicstyle=\ttfamily\scriptsize\bfseries,label={lst:grammar}]
S = scene
$\Sigma$ = {$\mathbb{N}, \mathbb{R}$}
N = {weather_index, global_road_friction, transform, perturbation, vehicle_color, vehicle_type, speed, trigger_distance, avoid_collision, after_trigger_behavior, travel_distance, pedestrian_type, static_type}
R = {scene -> background + ego_car + objects | $\epsilon$

    background -> weather_index + global_road_friction
    ego_car -> path
        path -> start_transform + middle_transforms + end_transform
            start_transform -> transform
            end_transform -> transform
            middle_transforms -> middle_transform + middle_transforms | $\epsilon$
                middle_transform -> transform + perturbation
    objects -> objects + vehicle | pedestrian | static | $\epsilon$
        vehicle -> vehicle_setup + vehicle_event
            vehicle_setup -> vehicle_color + vehicle_type + spawn_transform + vehicle_initial_speed
                spawn_transform -> transform
                vehicle_initial_speed -> speed
            vehicle_event -> waypoint_follower | going_straight | $\epsilon$
                waypoint_follower -> trigger_distance + target_waypoint + target_speed + avoid_collision + after_trigger_behavior | $\epsilon$
                    target_waypoint -> transform
                    target_speed -> speed
                going_straight  -> trigger_distance + target_speed + travel_distance + after_trigger_behavior
        pedestrian -> pedestrian_setup + pedestrian_event 
            pedestrian_setup -> pedestrian_type + spawn_transform
            pedestrian_event -> trigger_distance + target_speed + travel_distance + after_trigger_behavior | $\epsilon$
        static -> static_type + spawn_transform
    }
\end{lstlisting}


\begin{lstlisting}[float,caption={An example of a leading car scenario in AutoFuzz},captionpos=b,frame=single,belowskip=0pt,label={lst:leading_car_example},language=Python]
'Town05_right_0': {
    'town_name': 'Town05',
    'direction': 'right',
    'route_id': 0,
    'location_list': [(-120, 25), (-103, 4)]
    }

'leading_car_braking': {'customized_parameters_bounds':{
        'num_of_static_min': 0,
        'num_of_static_max': 0,
        'num_of_pedestrians_min': 0,
        'num_of_pedestrians_max': 5,
        'num_of_vehicles_min': 1,
        'num_of_vehicles_max': 2,

        'vehicle_x_min_0': -0.5,
        'vehicle_x_max_0': 0.5,
        'vehicle_y_min_0': -3,
        'vehicle_y_max_0': -15,

        'vehicle_initial_speed_min_0': 3,
        'vehicle_initial_speed_max_0': 7,
        'vehicle_targeted_speed_min_0': 0,
        'vehicle_targeted_speed_max_0': 3,
        'vehicle_trigger_distance_min_0': 3,
        'vehicle_trigger_distance_max_0': 15,

        'vehicle_dist_to_travel_min_0': 5,
        'vehicle_dist_to_travel_max_0': 30,
        'vehicle_yaw_min_0': 270,
        'vehicle_yaw_max_0': 270
    },
    'customized_parameters_distributions':{
        'vehicle_x_0': ('normal', None, 1),
        'vehicle_y_0': ('normal', None, 8)
    },
    'customized_center_transforms':{
        'vehicle_center_transform_0': ('waypoint_ratio', 0)
    },
    'customized_constraints':[
    {'coefficients': [1, 1],
    'labels': ['vehicle_trigger_distance_0', 'vehicle_y_0'],
    'value': 0}
    ]}
\end{lstlisting}



\subsection{Route}
A user needs to specify manually a seed route the ego-car should run. In particular, a list of locations (x, y) with length at least two should be given for the field \textit{location\_list}. The first and last element of the list will be the start location and destination of the ego-car. The user also needs to specify \textit{town\_name} corresponding to the map used. The field \textit{direction} and \textit{route\_id} are mainly for the purpose of folder creation. The field \textit{direction} corresponding to the direction the ego-car will go if it follows the route. The field \textit{route\_id} is an index number used to differ one route from the other.  

A user also needs to specify the search range and distribution of each feature. For the fields that are not specified, default values will be used. For a field with label "label", the user can usualy specify its range via label\_min and label\_max. If the field belongs to the i-th object of a category, that range is usually label\_min\_i and label\_max\_i. For simplicity of notation, we aggregate this pair of value with the notation label\_min/max. For the i-th object, we denote its range to be label\_min/max\_i.


\subsection{General and Ego-car}
There are 21 predefined weather modes, each of them consists of a setup of the weather(e.g. rain, fog) and lighting condition(e.g.noon, afternoon, night). They can be edited and more can be added if needed. Users can also set the search range of the friction of all roads via \textit{friction\_min/max}. Uers can control the range of the number of vehicles, pedestrians and static objects via \textit{num\_of\_static\_min/max}, \textit{num\_of\_pedestrians\_min/max}, and \textit{num\_of\_vehicles\_min/max}, respectively.

The first five interpolated waypoints of the vehicle can be perturbed. The perturbation range of the \textit{j}-th waypoint is controlled by \textit{perturbation\_x\_min/max\_j} and \textit{perturbation\_y\_min/max\_j}.

\subsection{Vehicle}
For a vehicle with index \textit{i}, the search ranges of x-axis and y-axis of its initial location, its facing direction and its initial speed can be specified by \textit{vehicle\_x\_min/max\_i},  \textit{vehicle\_y\_min/max\_i}, \textit{vehicle\_yaw\_min/max\_i}, and \textit{vehicle\_initial\_speed\_min/max\_i}, respectively. It can be triggered when the ego-car is within certain distance. The search space of this trigger distance is defined by \textit{vehicle\_trigger\_distance\_min/max\_i}. When the vehicle gets triggered, it has two potential behaviors: waypoint follower or going straight. The behavior is controlled by a binary variable \textit{is\_waypoint\_follower}. It can be set by the user by setting a range \textit{vehicle\_waypoint\_follower\_min/max\_i}. If the car is a waypoint follower, it follows CARLA interpolated route with a specified speed to a specified destination. The search range of x-axis and y-axis of its targeted destination can be controlled via \textit{(vehicle\_targeted\_x\_min/max\_i} and \textit{ (vehicle\_targeted\_y\_min/max\_i}, respectively. It can also be chosen to avoid collision or not. 

That range can be controlled via \textit{vehicle\_avoid\_collision\_min/max\_i}. If the car is going straight, it goes along a certain direction with a certain speed for a specified distance. The range o the distance it will travel is controlled by \textit{vehicle\_dist\_to\_travel\_min/max\_i}. The range of the direction it will go is controlled by \textit{vehicle\_targeted\_yaw\_min/max\_i}. The speed search range for both triggered behaviors can be set via \textit{vehicle\_targeted\_speed\_min/max\_i}.

The first five interpolated waypoints of the vehicle can be perturbed. The perturbation range of the \textit{j}-th waypoint is controlled by \textit{vehicle\_i\_perturbation\_x\_min/max\_j} and \textit{vehicle\_i\_perturbation\_y\_min/max\_j}.

Lastly, the available \textit{vehicle\_types} and \textit{vehicle\_color} can be modified or added.


\subsection{Pedestrian}
For a pedestrian with index \textit{i}, the search ranges of x-axis and y-axis of its initial location, and its facing direction can be specified by \textit{pedestrian\_x\_min/max\_i},  \textit{pedestrian\_y\_min/max\_i}, and \textit{pedestrian\_yaw\_min/max\_i}, respectively. It should be noted that pedestrians are initiated to be static and will move only when triggered. The search range of its triggered distance, its speed, and the distance it will travel are governed by \textit{pedestrian\_trigger\_distance\_min/max\_i}, \textit{pedestrian\_initial\_speed\_min/max\_i} and \textit{pedestrian\_dist\_to\_travel\_min/max\_i}, respectively.

Lastly, \textit{pedestrian\_types} can be modified or added.  

\subsection{Static}
A static object can be any stationary object (e.g. trashcan, barrel) that might appear on the road or nearby. For a static object with index \textit{i}, the search ranges of x-axis and y-axis of its initial location, and its facing direction can be specified by \textit{pedestrian\_x\_min/max\_i},  \textit{pedestrian\_y\_min/max\_i}, and \textit{ pedestrian\_yaw\_min/max\_i}, respectively.

Its available \textit{static\_types} can also be modified.

\subsection{Distribution}
For each of the aforementioned real value, a clipped distribution can be defined. The name used to control distribution is same except not having "min" or "max". For example, if a user can set the x-axis of the 0-th vehicle to be normally distributed with mean 0 and variance 1 by letting \textit{vehicle\_x\_0} to have value \textit{('normal', 0, 1)}, where the first field is the distribution's name and the second and last terms are mean and variance, respectively. Note that the mean value can be assigned "None", in which case, the mean value of the lower and upper bound of the field will be used.

\subsection{Center Transform}
It should be noted that for easier search process we center the location values by 0. However, we need to set a center for it. By default, the center is the middle waypoint of the interpolated routes. A used can change the center of an object with index \textit{i} by setting the value of \textit{<object\_type>\_center\_transform\_i} to be either ('waypoint\_ratio', percentage) or ('absolute location', x, y), where the former is an interpolated waypoint along the planned route corresponding to that percentage from the starting location and the later is explicitly specifying the location.

\subsection{Constraints}
Constraints between fields can also be specified. The constraints allow users to have greater flexibility when customizing their scenes. For example, a user may want at the starting of a scenario, the distance between the ego-car and a car in front of it to be larger than a certain distance to give ego-car enough time to react. Another example can be a user may want the speed of a leading car to be larger than its speed after triggering when trying to create a leading car slowing down scenario. When customized constraints are specified, sampling will only sample data satisfying these constraints and simulation will only be run when the scene satisfies the constraints. To specify constraints, the user provides a list of them. For each constraint, three fields need to be specified. The first field 'coefficients' is a list of coefficients to be multiplied before each of the selected feature. The field 'labels' is a list of features that participate in this constraint. Finally, a 'value' on the right-hand side needs to be specified. 

\subsection{Example: leading car deacreasing speed}
Listing \ref{lst:leading_car_example} shows a customized specification for an instance of the motivated scenario shown in Figure \ref{fig:scenario_demo}. In this case, the user wants to first specifies the search range for the number of static objects, pedestrians, and vehicles to be 0, [0,5], and [1,2], respectively. Note since the user wants to have a leading vehicle, the lower bound of the number of vehicles should be at least 1. Assume the vehicle with index 0 is considered to be the leading vehicle. The user limits the range of its spawn location such that it is ahead of the ego-car and on the same road. To achieve this, the range of the x-axis and y-axis are set to be (-0.5, 0.5) and (-3, -15) with center to be the initial location of the ego-car (("waypoint\_ratio", 0) is set to achieve this). The direction of the vehicle 0 is set to be 270 degrees. It must be noted that the reason that the range of the y-axis is negative and its facing direction are all chosen based on the route and the map. Further, the user may want the distribution of the values over the ranges to be normal rather than uniform and achieve this by setting \textit{vehicle\_x\_0} and \textit{vehicle\_y\_0} to be ('normal', None, 1) and ('normal', None, 8). With the second field to be None, the mean of the normal distribution is set to be the mean value of the range i.e. 0 and -9, respectively. 

Next, the user sets the range of the initial speed of the vehicle 0 to be [3, 7] and the speed after being triggered to slow down to be [0, 3]. The slowing down gets triggered when the ego-car is within [3, 15] of the vehicle 0. The traveling distance after slowing down is [5, 30].

With these specification, scenarios similar to \ref{fig:scenario_demo} will be generated and run by the simulator. Buggy cases will be reported and the \tool will also keep generating more potential buggy scenarios based on the feedback of the simulations.

Finally, the user may not want the leading vehicle to slow down at the beginning of the simulation. This is controlled by the specified customized constraint, where the trigger distance of vehilce 0 is constrained to be smaller than the vehicle 0's distance with the ego-car (since the center is the ego-car's location, the y-axis value of the initial location of vehicle 0 is equal to the initial distance between the ego-car and the vehicle 0).






\section{Methodology}
\subsection{Overview of \tool}
Figure \ref{fig:autofuzz_flowchart} gives a high-level overview of how high-level \tool works. A user first provides the controller under test and specifies a map and a seed route as well as the search space and distribution of each feature. \tool uses these information to sample the initial scenes. The simulator run these scenes, report found bugs and provide feedback to \tool. \tool leverages the feedback to generate more scenes. In the rest of this section we will formulate the search process as a constrained multi-objective optimization problem and provides details of solving it.

\begin{figure}[ht]
\centering
% url: https://drive.google.com/file/d/1MsJnf8ca4jks5KlUS5BHajweH8vFJ3XT/view?usp=sharing
\includegraphics[width=0.48\textwidth]{images/general/AutoFuzz_flow.pdf}
\caption{An illustration of how AutoFuzz works.}
\label{fig:autofuzz_flowchart}
\end{figure}




\subsection{Definition of Bugs}

\noindent\textbf{Bug Types}\\
There are many kinds of abnormal behaviors a self-driving car can potentially has \cite{}. In this work, we mainly focus on two types of errors: collision and out-of-road since these two can lead to serious consequences and also commonly studied in the literatures \cite{}. However, our framework can be easily extended for other types of errors e.g. running a red traffic light. 

A collision error consists of collision with other vehicles, collision with cyclists/motorcycles, collision with pedestrians, or collision with stationary objects like a trash can or a road boundary. A out-of-road error consists of going to a wrong lane (a lane that has opposite traffic direction that the car drives towards) and going off road. We will later present how we formulate objectives to promote finding such errors.

\noindent\textbf{Uniqueness of Bugs}\\
Defining distinct bugs in self-driving car controller is a very hard problem. Bugs in self-driving car controller are different from traditional software bugs. Because there are many dimensions of the input parameters being continuous, there can be infinitely "different" bugs. For example, the existence of a static object (say, a barrel) in front of a car causes a crash. By modifying other input parameters (e.g. the position of another pedestrian, the color of another vehicle etc.) that are unrelated (e.g. they may not be seen by the ego-car), we can get an infinite number of "different" bugs that provide little extra information. Thus, we propose a criteria that allow us to only count real unique bugs.
In \cite{testing_vision18}, they define that two test scenarios are distinct if they differ in "the value of at least one static variable or in the value of at least one dynamic variable with a significant margin." This definition fails in our more complex scenarios as my example will be considered different bugs by their creteria. To avoid counting similar bugs as different bugs, we give a definition that gives a "lower bound" of the number of bugs by binning them.


 we define two bugs A and B being different if their they have more at least 50\% fields being different (for discrete fields) or different by a large margin (for continuous fields). In the experiment part, we define two bugs A and B being different if their they have more at least 50\% fields being different (for discrete fields) or different by a large margin (we choose 15\% for continuous fields).


\subsection{Finding Bugs as Multi-Objective Optimization}
We formulate the problem of finding failure cases as a constrained multi-objective optimization problem. It should be noted that although \cite{testing_vision18} also formulates the problem as a multi-objective search problem, we have completely different purposes. Here, our objectives are designed to make a self-driving car controller to violate different types of errors, while in \cite{testing_vision18}, their objectives are all for fooling the particular Automated Emergency Brake system.  Denote $x\in \mathbb{R}^k$ to be a scene vector that consists of all the specified search-able variables. Denote $f_i(x):\mathbb{R}^k \rightarrow \mathbb{R}$ for $i=i,...,m_1$ to be $m_1$ objective functions. Denote $g_j(x):\mathbb{R}^k \rightarrow \mathbb{R}$ for $j=j,...,m_2$ to be $m_2$ constraint functions that must be less than or equal to 0. The optimization has the following form:
\begin{align*}
    \textrm{min}_x~ & \sum_{i=1}^{m_1} f_i(x) \\ 
    \textrm{s.t. } & g_j(x) \leq 0 ~\forall j=1,...,m_2
    \label{eq:optimization}
\end{align*}
There are many kinds of algorithms we can potentially use to solve it e.g. multi-objective genetic algorithms \cite{}, bayes optimizations \cite{}. In this work, we mainly focus on NSGA2 \cite{} and NSGA2-DT \cite{}, as they have been shown to be effective on a smaller-scale similar error finding optimization problem. We argue that our framework can be easily extended to also support other multi-objective optimization algorithms.



\noindent\textbf{objective function}\\
It is very important to formulate the objective functions since they usually determine if the algorithm can successfully find the bugs. We define the following objective functions:
\begin{align*}
    f_{v-collision} &:= \textrm{speed of ego-car at collision} \\
    f_{d-object} &:= \textrm{minimum distance to other objects} \\ 
    f_{d-wronglane} &:= \textrm{minimum distance to an opposite lane} \\
    f_{d-offroad} &:= \textrm{minimum distance to a non-drivable region} \\
    f_{d-deviation} &:= \textrm{maximum deviation from interpolated route}
\end{align*}
All of these functions are continuous for a smooth improvement of the search algorithm. In particular, the first two, $f_{v-collision}$ and $f_{d-object}$, promotes collision error. Note a special case of $f_{d-object}$ is the minimum distance between either of the front two corners of the ego-car's bounding box and any other object's corner of bounding box. This special case can be used for testing controllers that only have front camera(s) since it might not be fair to test out-of-sight collision which goes beyond their assumed capability. They promote the severity of collision and the chance of collision, respectively. The rest three promotes out-of-road error. $f_{d-wronglane}$ promotes going to wrong lane and $f_{d-offroad}$ promotes going off road, while $f_{d-deviation}$ promotes both. It should be noted that for $f_{d-wronglane}$ and $f_{d-offroad}$, we find a directed version. 
Figure \ref{fig:wronglane_objective} shows a car driving along a road. Its forward direction is denoted as v, its direction and distance with respect to the closest point that is on a road with different direction compose another vector d, and the angle between the two vectors is denoted as $\theta$ (in radian). $f_{d-wronglane}$ is equal to $||d||_2\times (1-\frac{2\times\theta}{\pi})$. $f_{d-offroad}$ is defined similarly except the closest point will be the one that is off road rather than on a opposite direction road.


\begin{figure}[ht]
\centering
% url: https://drive.google.com/file/d/1MsJnf8ca4jks5KlUS5BHajweH8vFJ3XT/view?usp=sharing
\includegraphics[width=0.3\textwidth]{images/general/wronglane_objective.pdf}
\caption{An illustration of the calculation of the wrong lane objective $f_{d-wronglane}$.}
\label{fig:wronglane_objective}
\end{figure}


\noindent\textbf{constraints}\\
There are two kinds of constraints: individual variable constraints and joint constraints. For each field $x_i$, its individual constraints is defined as its possible minimum and maximum values. Each joint constraints is defined as an inequality equation $\sum_{i\in \mathbf{S}} c_i \times x_i \leq v$, where $S$ is a subset of all features, $c_i$ is a real number coefficient, and $v$ is a real value. Users can specified both as discussed earlier. \tool will respect both but in a different way. It will clip the values for individual variable constraints' violations, while it will avoid running simulation for cases that violate joint constraints.




\subsection{Algorithm}
We adapt the Non-dominated Sorting Genetic Algorithm version 2 (NSGA-2) \cite{nsga2} algorithm, which is a widely used evolutionary multi-objective search algorithm and also used in \cite{testing_vision18} for our framework. Algorithm \ref{alg:ga-un} shows our algorithm NSGA2-UN. It worth noting that it is easy to extend our framework to support other algorithms.

\noindent \textbf{Initial Population}: For generating one instance, we randomly sample each variable according to its user specified search range and distribution. If the specified constraints are not satisfied, each variable will be re-sampled. If the specified constraints have very few small probability and cannot be satisfied after trying a specified number of attempts, the program will stop and raise an error.

\noindent \textbf{Fitness Functions}: We use the summation of the objective functions defined in the earlier section as the fitness function. The weights can be adjusted according to a user's need. For example, if the user only wants to focus on finding collision errors, the last three weights can be set to 0.

\noindent \textbf{Selection}: We adopt binary tournament selection with replacement which is used in both the original implementation of NSGA-2\cite{nsga2}. It create two duplicates for each (since we only keep the population with initial population size e.g. 100)and randomly pair up these new samples. It chooses the winner of each pair and randomly pair up these winners as the parents for this generation's mating process. 

\noindent \textbf{Crossover}: Simulated Binary Crossover \cite{SBX}, a classical crossover method that is commonly used to float variables is adopted. A distribution index ($\eta$) is used to control the similarity of the offsprings and their parents. The larger $\eta$ is, the more similar the offsprings are with respect to their parents. We set $\eta=20$ as the same as \cite{testing_vision18}.

\noindent \textbf{Mutation}: Polynomial Mutation is applied to each variable \cite{polymutation} for both discrete and continuous variables. For discrete variable, we treat the value as continuous during the mutation and round them afterwards. We clip the values at specified minimum and maximum values. Following \cite{testing_vision18}, mutation rate is set to $\frac{1}{k}$, where $k$ is the number of variables an instance has. The mutation magnitude is controlled by a variable $\eta_m$. Based on \cite{polymutation}, $\eta_m$ usually induces an effect of a perturbation $O(\frac{x_{i_{max}}-x_{i_{min}}}{\eta_m})$, where $x_{i_{max}}$ and $x_{i_{min}}$ are the upper and lower bounds of a variable $x_i$, and a value of $[20, 100]$ is usually adequate. In this work, we set $\eta_m=20$. 

\noindent \textbf{Duplicates Elimination}: 
Note that after each selection, crossover, and mutation, the proposed offspring are filtered out if they are similar to any of previous found bugs. The process will repeat until the number of offspring reaches the number of desired population size or maximum number of iterations reaches.

\noindent \textbf{Survival}
We use NSGA2's default survival strategy, rank and crowding survival, and only keep the initial population size (i.e. we cut off half of data from the parents and offspring combined set). It first non-dominated sort the data, it then include front by front until coming to a front that it has to split. It take the elements of that particular front based on crowding score.

% $l_p$-norm distance (after normalization of each continuous field and counting discrete field difference as t ($0\leq t\leq 1$) which trades off importance of continuous and discrete field)) is larger than a threshold value $th$.

    



\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{evaluate(), max-gen, pop-size, max-mating-iter}
    \Output{unique-bugs}
    
    generations = 0\;
    unique-bugs = []\;
    
    current-population, current-objectives = sampling(pop-size)\;
    offspring = current-population\;
    
    \While {generations < max-gen}{
        generations += 1\;
        new-unique-bugs, new-objectives = evaluate(offspring, unique-bugs)\;
        
        unique-bugs = merge(unique-bugs, new-unique-bugs)\;
        combined-population = merge(current-population, offspring)\;
        combined-objectives = merge(current-objectives, new-objectives)\;
        
        current-population, current-objectives = survival(combined-population, combined-objectives, pop-size)\;

        mating-iter = 0
        offspring = []\;
        remaining-size = pop-size\;
        \While {mating-iter < max-mating-iter and remaining-num > 0}{
            mating-iter += 1\;
            parents = selection(current-population, remaining-num)\;
            new-offspring = crossover(parents)\;
            new-offspring = mutation(new-offspring)\;
            new-offspring = filtering(new-offspring, offspring, unique-bugs)\;
            
            offspring = merge(offspring, new-offspring)\;
            remaining-num = pop-size - len(offspring)\;
        }
        \If {len(offspring) < pop-size}
        {
            remaining-num = pop-size - len(offspring)
            remaining-offspring = sampling(remaining-num)\;
            offspring = merge(offspring, remaining-offspring)\;
        }
        
    }
    
    
    \Return unique-bugs
    

    \caption{NSGA2-UN}
    \label{alg:ga-un}
\end{algorithm}
